SAQIEL: Ultra-Light and Safe Manipulator with Passive 3D Wire Alignment Mechanism

Improving the safety of collaborative manipulators necessitates the reduction of inertia in the moving part. Within this paper, we introduce a novel approach in the form of a passive 3D wire aligner, serving as a lightweight and low-friction power transmission mechanism, thus achieving the desired low inertia in the manipulator's operation. Through the utilization of this innovation, the consolidation of hefty actuators onto the root link becomes feasible, consequently enabling a supple drive characterized by minimal friction. To demonstrate the efficacy of this device, we fabricate an ultralight 7 degrees of freedom (DoF) manipulator named SAQIEL, boasting a mere 1.5 kg weight for its moving components. Notably, to mitigate friction within SAQIEL's actuation system, we employ a distinctive mechanism that directly winds wires using motors, obviating the need for traditional gear or belt-based speed reduction mechanisms. Through a series of empirical trials, we substantiate that SAQIEL adeptly strikes balance between lightweight design, substantial payload capacity, elevated velocity, precision, and adaptability.

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag} % 古いコマンドやパッケージの利用を警告する
\usepackage[all, warning]{onlyamsmath} % amsmath が提供しない数式環境を使用した場合に警告
% not for arxiv
% \usepackage[dvipdfmx]{color}
% \usepackage[dvipdfmx,bookmarks=true,bookmarksnumbered=true,bookmarkstype=toc,%
%      colorlinks=true,%
%      linkcolor=black, %%追加20090108
%      citecolor=black, %%追加20090108
%      urlcolor=black, %%追加20090108
%      bookmarksopen=true,%しおりツリーをデフォルトで開く
% %     backref=page,%citeにどこで使っているか出るようになる
%      pdftitle=\PDFTITLE,%
%      pdfsubject=\PDFSUBJECT,%
%      pdfauthor=\PDFAUTHOR,%
%      pdfkeywords=\PDFKEYWORDS]{hyperref}
% %% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvips]{graphicx}
% \usepackage[dvipdfmx]{}
% \usepackage{jtygm}
% \usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
% for arxiv
\usepackage{hyperref}
\usepackage{color}
\usepackage{graphicx}

\usepackage{url}

\usepackage{txfonts,mathptmx}

%%%% カスタマイズしたい場合は以下に書く

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}

% \usepackage{pxjahyper}
% hypcap: figref, tabrefしたときにジャンプ先がキャプション部ではなく図の上になる
\usepackage[figure,figure*,table,table*]{hypcap}
% \usepackage{eclbkbox}
%% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvipdfmx]{}
% \usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
%\usepackage{html} % latex2html で 利用
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}
\usepackage{siunitx}
\usepackage{booktabs}
\usepackage{lscape}
\algblockdefx{FORP}{ENDFORP}[1]%
  {\textbf{for}#1 \textbf{do in parallel}}%
  {\textbf{end for}}
\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}

%% \newcommand{\tabref}[1]{{表~\ref{#1}}~}
%% \newcommand{\figref}[1]{{図~\ref{#1}}~}
%% \newcommand{\equref}[1]{{式(\ref{#1})}~}
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\subsecref}[1]{Subsection \ref{#1}}
\newcommand{\tabref}[1]{{Table. \ref{#1}}}
\newcommand{\figref}[1]{{Fig. \ref{#1}}}
%% \newcommand{\figref}[1]{\figurename\ref{fig:#1}}
\newcommand{\equref}[1]{{Eq. \ref{#1}}}
\newcommand{\algoref}[1]{{Alg. \ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}
%% \renewcommand{\figurename}{Fig.}
%% \renewcommand{\tablename}{Table }

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}


